Behavioral Program Logic and LAGC Semantics without Continuations (Technical Report)

We present Behavioral Program Logic (BPL), a dynamic logic for trace properties that incorporates concepts from behavioral types and allows reasoning about non-functional properties within a sequent calculus. BPL uses behavioral modalities [s |- {\tau} ], to verify statements s against behavioral specifications {\tau}. Behavioral specifications generalize postconditions and behavioral types. They can be used to specify other static analyses, e.g., data flow analyses. This enables deductive reasoning about the results of multiple analyses on the same program, potentially implemented in different formalisms. Our calculus for BPL verifies the behavioral specification gradually, as common for behavioral types. This vastly simplifies specification, calculus and composition of local results. We present a sequent calculus for object-oriented actors with futures that integrates a pointer analysis and bridges the gap between behavioral types and deductive verification. This technical report introduces (1) complete LAGC semantics of a Core Active Object language (CAO) without continuations (2) Behavioral Program Logic and (3) gives an example for a behavioral type expressed in Behavioral Program Logic, method types. This report contains the soundness proofs for method types. While the semantics cover CAO with suspension, the method types do not, to simplify the presentation.

==> chapters/034_discuss.tex <==
\subsection*{On the Design and Limitations of \coreactor}
\paragraph{Object Creation.}
Object creation is restricted in \coreactor: the main block uses Rebeca-style initialization and one asynchronous method call and dynamic object creation is not allowed.
The reason for this design decision requires a discussion of some concepts of the later Chapter~\ref{ch:st}: 
Session Types for Active Objects so far lack the ability to assign roles to newly created objects, e.g., by role delegation~\cite{DenielouY11}, which is used in Session Types for channel-based concurrency models.
Furthermore, channel-based concurrency models isolate a session by grouping a set of process by a shared channel. The session is thus \emph{isolated} from the rest of the system, but processes may participate in multiple sessions~\cite{BocchiDY12}.
It is harder to isolate sessions without channels, especially if the concurrency model allows interactions via the heap memory. 
As it is out of scope for this work to lift all possible extensions of Session Types from channel-based concurrency models to Active Objects, we regard the whole system as one session. 
Din et al.~\cite{DinSC18} isolate sessions in Active Objects, but introduce a new transaction mechanism to enforce isolation at runtime, while this work gives a fully static system.


We give a discussion of the semantics of dynamic object creation their possible treatment by method contracts and object invariants, and a discussion on runtime enforcement in \EK{later Chapters}.

\paragraph{Runtime Errors.}
Our language does not include exceptions. In contrast, ABS has three implicitly thrown exceptions  \abs{NullPointerException}, \abs{PatternMatchException}, \abs{DivisionByZeroException}:
\begin{itemize}
\item \abs{NullPointerException}. In \coreactor, all locations of class type are initialized at program start with non-null values. As there is no \abs{null} constant, it is not possible to raise such an exception.
\item \abs{PatternMatchException}. This is thrown by the functional sub language of ABS when a deconstruction of an value with a abstract data type(ADT) is not possible. 
\item \abs{DivisionByZeroException}. This exception is self-explaining.
\end{itemize}
\coreactor has only the \abs{List} ADT, so runtime errors can only occur by evaluating \abs{head(Nil)} and \abs{e/0}.
In this case the evaluation is not defined, no rule can be applied and thus the object blocks.  

The reasoning system we present in the following chapters is only concerned about \emph{partial} functional correctness: correctness in case of normal termination~\cite{BeckertK016}. Thus, the ramifications of exception handling would offer no insights.
Furthermore, their treatment in dynamic logic is well-explored. Excluding them vastly simplifies the assignment rules for symbolic execution, because there is no need for program transformation that ensure that the right-hand-side of assignments is a s non-nested expressions. 

We discuss exceptions and the effect of program transformations in \EK{later Chapters}.

\subsection*{On the LAGC Semantics}
Compared to the original formalization of Din et al.~\cite{DinHJPT17}, we have made some adaptations. 

The biggest difference is that we have no continuations. Din et al. use such special markers at points where input is required, instead of using fresh symbolic values and similarly, other markers to mark processes as starving or blocked. 
These markers are used to control interleavings in the external semantics, which have only two layers (method local, system global) instead of three (method local, object local system global) and always add as much of a local trace as possible.
We replaced this with our agreement mechanism that chops up a trace step by step.

With continuations, the semantics of a method is less clear and the resulting traces are harder to reason about (in the sense that they are not straightforward models for our semantic logics).
For example, the semantics of \abs{v = f.get; if(v>0) { i=v }else { i=-v}; return i} has two traces in our semantics, one for each branch of the \abs{if} statement.
Din et al. have three traces: two traces for the branches of the \abs{if} statement, in case that the future in \abs{f} has already been resolved, and one trace of the following form for the case that it is not\footnote{We refrain from using the original syntax for readability's sake}:
\scalebox{0.9}{\begin{minipage}{\textwidth}
\[\emptyset \triangleright \sequence{\defstatepair,\mathit{blkEv}(\objname,\defeval{f}),\mathit{blkCont}(\objname,\destiny,\xabs{v = f.get; if(v>0) { i=v }else { i=-v}; return i})}\]
\end{minipage}}

The continuation marker $\mathit{blkCont}$ is used to generate further local traces (here: two more, thus four traces in total, despite the statement having only two branches) by the global semantics. 
Thus, local and global semantics are not clearly separated. 
However, there is no need for the more complex handling of symbolic fields in our system: the fresh symbolic heap during generation can be seen as generating the continuations already at that point. 

Din et al. do not discuss selectability, which we propose is easier with our approach than with continuations. 
We also do not model starvation explicitly. Instead of adding a starvation marker to the local semantics, it is modeled explicit as a process that is never scheduled again. 
We propose that starvation is a property that is visible at object level and should, thus, not be modeled at method level. Our approach is also nearer to the definition of starvation used by static analyses~\cite{avocs}.

Finally, we do not use a well-formedness predicate to ensure that basic consistency conditions are uphold, e.g., that a method starts only after it is called. 
The only places where explicit checks are needed are to ensure future freshness and that the correct value is read from a future.
\subsection*{On the Semantic Logics}
We stress that both MSO logics are \emph{not} MSO over finite words, because we include semantic values into the structure. 
Thus, they are equally expressive not to the $\mu$-calculus, but to Quantified CTL$^\ast$~\cite{LaroussinieM14}\footnote{Under certain restrictions on the structure, we refer to Larousinie et al.~~\cite{LaroussinieM14} and David et al.~\cite{DavidLM16} on a discussion on this topic, and refrain from a detailed discussion in this work as the expressive power of the semantic logics offers no insights into the further reasoning framework.}.
Furthermore, relativization for MSO is straightforward and quantifiers make it easier to express global properties (i.e., properties that relate potentially far away parts of the trace). 
As we give not calculus for the semantic logics, their choice is mainly a matter of preference and the use of full second order logic or a temporal logic is also possible in principle.

